Gender Disparity in Publishing Six Months after the KITP Workshop "Probes of Transport in Stars"

Conferences and workshops shape scientific discourse. The Kavli Institute for Theoretical Physics (KITP) hosts long-term workshops to stimulate scientific collaboration that would not otherwise have taken place. One goal of KITP programs is to increase diversity in the next generation of scientists. In this analysis, we examine gender trends in authorship of papers generated as a result of the KITP program \textit{Probes of Transport in Stars}, which ran from October 11th, 2021 to December 17th, 2021. While 38\% of workshop participants were women, only 19\% of publications produced between December 1st, 2021 and June 3rd, 2022 had female first-authors. Further, of these early publications, 61\% had all-male author lists. Among publications resulting from the KITP program, the proportions of both male first-author papers and papers with all-male author lists are higher than predicted by models that take into account the gender distribution of the KITP participants. These results motivate more thorough investigations of collaboration networks at scientific conferences and workshops. Importantly, they also suggest that programs, conferences, and workshops of any kind need to take steps beyond those implemented in this KITP program to enable more diverse collaborations and address gender disparities in science.

==> Jamies_notes.tex <==
%%% Abstract
% In the roughly six months since the 
% %\sout{first day} 
% final week of the KITP program \textit{Probes of Transport in Stars}, 45 in-person participants led or were included as authors on a total of 94 scientific contributions shared to the arXiv and searchable on NASA ADS. Here, we briefly examine the gender breakdown of the author lists among this set of publications.
% %
% We find that the ratio of male-led to female-led \textit{KITP publications} is significantly greater than the ratio of male to female participants, as is the ratio of total male authorships to total female authorships.\pink{``We find that both the ratio of male-led to female-led \textit{KITP publications} and the ratio of total male authorships to total female authorships are significantly greater than the ratio of male to female participants.'' Or maybe: ``We find that \textit{KITP publications} were disproportionately led by men, and men have disproportionately-many total authorships'' Could improve upon the second phrase.} We also find that women are more likely to have female co-authors than men, and that male-led papers are exceedingly more likely to have single gender (all male) author lists than author lists that contain even a single woman. Further, the data encourage speculation as to differences in use of KITP time as a function of gender, with men devoting more time to new projects and collaborations and women ``playing catch up'' on pre-KITP projects.
% %
% Collectively, these statistics paint a portrait of KITP as a productivity goldmine, but one from which men clearly benefit more---or, at least, more quickly---than women.

%%%% Intro

% Evidence seems to indicate that scientists that collaborate are more productive (Kyvik S, Teigen M. 1996, Jadidi2017 and references therein).}
%KatzMartin1997: Research into this question seems to indicate that high productivity (in terms of published output) is indeed correlated with high levels of collaboration [1-4,24,30,51,52,58,60]. 
%For example, the centrality of a scientist in a collaboration network isassociated with her success [51,52], and co-authorship strength is related to highproductivity and citations [43,44]
%[43]  Petersen, A. M., Quantifying the impact of weak, strong, and super ties in scienti ̄ccareers,Proc. Natl. Acad. Sci. USA112(2015) E4671–E4680.[44]  Petersen, A. M., Fortunato, S., Pan, R. K., Kaski, K., Penner, O., Rungi, A., Riccaboni,M., Stanley, H. E. and Pammolli, F., Reputation and impact in academic careers,Proc.Natl. Acad. Sci. USA111(2014) 15316–15321.
%
% Previous works on scienti ̄c collaborationsuggest that men and women tend to exhibit di®erent collaborative behaviors acrosstheir scienti ̄c career, such as di®erences in the number of new and repeatingcollaborations [24,71], position in the network [64], degree of homophilic behavior[14,34] and tendency to have interdisciplinary collaborations [26,50]
%
%female scientists have signi ̄cantly fewer distinct co-authorsover their careers and a lower probability of repeating previous collaborations thanmales [71].
%
%However, there are a variety of different author relationships, including those that involve formal collaborations, those related to mentoring, as well as local and global connections. 
%need to see how common these terms are before committing to explaining them
%https://www.sciencedirect.com/science/article/pii/S0048733304000162?via%3Dihub


%(FerberTeiman1980, McDowellSmithKiholm1992,Jadidi2018) 
%\citep{BozemanCorley2004, RhotenPfirman2007, BozemanGaughan2011}.%(BozemanCorley2008, RhotenPfirman2007, BozemanGaughan2011).

%Child care, research collaboration, and gender differences in scientific productivity. Science, Technology & Human Values. 1996;21(1):54–71. https://journals.sagepub.com/doi/pdf/10.1177/016224399602100103) 


%Katz and Martin (1997) point out four key advantages of using co-authorship as a measure of collaboration including its verifiability, stability over time, data availability and ease of measurement. But they also note that co-authorship is no more than a partial indicator of collaboration. https://www.sciencedirect.com/science/article/pii/S0048733396009171

%External research collaboration in two small science systems Scientometrics, 49 (2000), pp. 145-160 
%https://www.scopus.com/record/display.uri?eid=2-s2.0-0005704429&origin=inward&txGid=a7c544bccfb4dc5e33a9e761ac76bb19&featureToggles=FEATURE_NEW_DOC_DETAILS_EXPORT:1

%Mary Frank-Fox has contended that we must consider how collegial interaction, work climate, collaborative opportunities, and institutional settings might affect the productivity rates of men and women in academic settings (Fox, 1991, Fox, 1985). Within academia, major decisions about rank, status, and position are typically decided in quite informal settings within the collegial network (Fox, 1991).

%(Kyvik S, Teigen M. 1996,Jadidi2018, although see also LeeBozeman2005)

%One especially interesting finding, not easily explained, is that tenure-track (but untenured) females have collaboration patterns almost identical to tenured males.

%One domain in which network science could offer insight is in the study of gender differences in authorship and collaboration patterns. Indeed, there have been several studies on this topic. For example, Araújo et al. (2017) analyzed a dataset containing more than 270,000 academics from a wide variety of fields (engineering, arts, biological, exact, and social sciences) in Brazil. They found that, across all fields, men were more likely to collaborate with other men, while for women, the gender ratio of their collaborations more closely matched that of the relevant academic population. In contrast, Karimi et al. (2018) showed that, in a research community in organizational science based in the US and Europe, women exhibited more gender homophily. Jadidi et al. (2018) investigated gender differences in a temporal network spanning 47 years with publication and citation data of over one million computer scientists, concluding that homophily has been increasing recently for both genders. Additionally, they found that women have a higher dropout rate than men, especially at the beginning of their careers. West et al. (2013) studied gender differences in a corpus containing over eight million publications in humanities, social and natural sciences. They found that, overall, gender differences in number of publications have been decreasing over time. However, in some fields, women remain disproportionately underrepresented as first, last, and solo authors.

%Studies of editorial decisions in leading journals in physics (Zuckerman and Merton 1971), in astronomy (Gordon 1980), in social psychology (Presser 1980), and in cancer research (Lawani 1986) show that joint-authored papers have a higher acceptance rate than do single-authored papers.

%Previous works on gender and collaboration [7, 12, 17, 23, 28] had information from a much smaller number of authors, usually much less than 10,000.

%lol In natural sciences, for example, the average number of article equivalents per faculty member is lower among older researchers than it is among younger ones, indicating that natural scientists have problems in keeping up with the research front as they become older (Kyvik 1990a).

%\pink{I think it would be useful to say more about why we're using this sample. Why not use a different sample of astrophysicists / a different time window? Is this about the effects of KITP on productivity for men vs women? General gender disparities in astrophysics?}
%\textbf{We use this dataset because we were close enough to the action to know what's going on...matter of convenience/closeness to the situation}



% This analysis considers a series of metrics quantifying the research productivity of scientists who participated in the Kavli Institute for Theoretical Physics (KITP) program \textit{Probes of Transport in Stars}, which ran from October 11th, 2021 to December 17th, 2021. It focuses in particular on trends with gender, where data (Section \ref{sec:data}) reveal that productivity signifiers for female participants, including publication rate, publication opportunities, and coauthorships, lag significantly behind those of male participants. In Section \ref{sec:results}, a preference among male participants for male collaborators is found, as is a large constituency of KITP publications with all-male \JB{KITP publications with only male KITP participants} author lists.

%% Section 2
%KITP strongly supports the inclusion of women and under-represented minorities in its programs and expects coordinators to make considerable efforts toward achieving this goal. We need you to designate one of  your Coordinators to be responsible as the Diversity Coordinator.    This person must be someone other than the lead point of contact for the program,


%Conference diversity:
%  - Speakers and session chairs should be broadly diverse (gender, under-represented groups, career stage, etc.).
%- Program diversity: Key thing is getting lots of applicants. Helps with inviting a diverse group.}

%Potential participants are required to apply for the program
%\sout{; during the selection process these applications were read, and statistics were kept on the applicant pool in general, the interests discussed in the application, and whether an applicant was likely part of an underrepresented minority}. 

%Please write a brief report that includes 1. A summary of the coordinators’ efforts to recruit scientists from underrepresented groups. 2. A list of applicants, developed by convening the coordinators and identifying appropriate scientists from underrepresented groups who have not yet applied. }
%As you assemble the speaker list, keep in mind that you must consider the inclusion of groups underrepresented in physics—we will monitor these efforts and ask for a summary as part of your final written report.  

%\sout{In the case of the Transport in Stellar Interiors conference, an unusual structure of review talks and panel discussions was adopted, with significant effort paid to include more junior researchers with a range of identities as speakers and panelists. During the conference itself, session chairs were reminded to be inclusive when calling on questioners, and provided with guidelines for inclusive chairing.} 
%https://www.sdss.org/collaboration/coins/coins-chairing-guidelines/


%%Section 4
% \pink{I thought we didn't want to comment on the gender of non-KITP participants, which is why we weren't considering the non-KITP authors in assigning all-male and all-female}


% So far, 18 scientific contributions classified as KITP publications have been publicly identified, of which 16 have a \textit{KITP author} as first author. Of the 18 overall, just over 83\% have a male first author 
% (whether that man is a KITP participant or not) compared to under 17\% with female first authors. 
% \pink{Also, I think these numbers are wrong... I met Amishi Sanghi at a conference and I think she's female. Don't know Hachem Dhouib, though google search suggests male.}
%% OK, good catch ^


% \pink{Similarly, I don't find the rest of this paragraph necessary}
% Although identifying individuals was a necessary part of obtaining the metrics presented here, we do not provide a breakdown of publication count by participant so as to avoid publicizing productivity statistics for individuals.\footnote{This is not necessary to draw our conclusions, nor is it in the best interests of young scientists in an already hyper-competitive culture to broadcast such information.} If the reader finds this information necessary, our data set can be reconstructed entirely from the public record. 

%%% 4.2

%  Of 18 KITP papers, 11 have all-male author \JB{KITP partipant instead of "author"?} lists, or 61\%. On the contrary, only two KITP papers have all-female author lists, and one of these is a single-author paper. Even including multi-gender papers, male-led coauthor lists show an overall 7:1 male-female ratio, on average. Restricting to the small number of female-led papers yields an average male-female ratio of 1:4, but this sample comprises (1) one female-led, single-author paper, (2) one paper with two female coauthors, and (3) one paper led by a female student and coauthored by her male supervisor. In addition to the small sample size, the coauthor configuration on each of the female-led publications deviates highly from the typical KITP paper (for example: the median number of coauthors for a general \textit{KITP paper} is 6 \textbf{[check this number]}, as compared to one or two coauthors for all female-led \textit{KITP papers}), so it is difficult to extract meaningful conclusions. The inverted gender ratio here is more likely a statistical coincidence.


%% 4.4

The number of male KITP participants who, as of June 3, 2022, have zero public contributions classified as \textit{KITP papers} is \textbf{about 50\%}. However, this number reduces to just \textbf{11\%} when \textit{KITP papers} and \textit{non-KITP papers} are considered. In contrast, the proportion of female KITP participants with zero \textit{KITP papers} is \textbf{65\%}, and the proportion of women with neither \textit{KITP papers} nor \textit{non-KITP papers} is 35\%---
just over one third of the total number of women. In other words, the vast majority of male participants \textbf{(89\%, or roughly 9 out of 10 men)} have had at least one publication opportunity on or before June 3, 2022, compared to less than two thirds of women (roughly 6 out of 10).

Relatedly, a greater proportion of total publications (all papers, KITP or non-KITP, published by a KITP participant after December 1, 2021) are \textit{KITP publications} for men than for women. For men, \textit{KITP publications} constituted 36\% of their overall research output during the time interval studied, compared to just 28\% for women.


%% section 5


% \textbf{[social science says that when you control for career stage, rates of publication among men and women are about the same for junior scientists, which makes our findings here even worse]}


% \textbf{[Meridith not here yet]}
% KITP programs were designed to be incubators for new ideas, but in practice they can also provide an otherwise rare opportunity for overburdened scientists to complete existing research free from academic service and home obligations. The data suggest that KITP served in the former function---as a hotbed for new pursuits---to a greater extent for men than for women.
\pink{Is this necessarily true? Maybe these papers were a result of men being able to complete existing research?}
%, and in the latter function---``catch up'' time---for women.  
The fact that the ``KITP research component fraction'' discussed in Section \ref{sec:research_frac} is more than 20\% higher for men than for women could have several explanations. Compelling among these is that men were better able to focus on new, KITP-related work during this time, whereas women were, on average, more preoccupied with existing projects. \textbf{[do social science citations go here?]}


% It is work noting that high publication rates were highly concentrated within a small number of individuals---mostly, but not entirely, male---and clearly reinforced by the fact that they were almost always coauthors on each other's publications.  

